Multi-Scale Supervised 3D U-Net for Kidneys and Kidney Tumor Segmentation

Accurate segmentation of kidneys and kidney tumors is an essential step for radiomic analysis as well as developing advanced surgical planning techniques. In clinical analysis, the segmentation is currently performed by clinicians from the visual inspection images gathered through a computed tomography (CT) scan. This process is laborious and its success significantly depends on previous experience. Moreover, the uncertainty in the tumor location and heterogeneity of scans across patients increases the error rate. To tackle this issue, computer-aided segmentation based on deep learning techniques have become increasingly popular. We present a multi-scale supervised 3D U-Net, MSS U-Net, to automatically segment kidneys and kidney tumors from CT images. Our architecture combines deep supervision with exponential logarithmic loss to increase the 3D U-Net training efficiency. Furthermore, we introduce a connected-component based post processing method to enhance the performance of the overall process. This architecture shows superior performance compared to state-of-the-art works using data from KiTS19 public dataset, with the Dice coefficient of kidney and tumor up to 0.969 and 0.805 respectively. The segmentation techniques introduced in this paper have been tested in the KiTS19 challenge with its corresponding dataset.

==> fig/xplot.tex <==
% This file was created by matplotlib2tikz v0.7.3.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.980392156862745,0.501960784313725,0.447058823529412}
\definecolor{color1}{rgb}{0.698039215686274,0.133333333333333,0.133333333333333}

\begin{axis}[
height=\figureheight,
legend cell align={left},
legend style={draw=white!80.0!black},
tick align=outside,
tick pos=left,
width=\figurewidth,
x grid style={white!69.01960784313725!black},
xmin=-18.25, xmax=383.25,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ymin=-0.00195300000000103, ymax=0.00747300000000044,
ytick style={color=black},
% ytick={-0.002,0,0.002,0.004,0.006},
% yticklabels={-0.002,0.000,0.002,0.004,0.006}
]
\addplot [semithick, color0, mark=*, mark size=0.3, mark options={solid}, only marks]
table {%
0 0
1 0.000239999999999997
2 0.00156
3 9.99999999999997e-06
4 0
5 -2.99999999999988e-05
6 -9.99999999999994e-05
7 -3.99999999999984e-05
8 -0.000210000000000002
9 -0.000150000000000001
10 -0.000129999999999998
11 -7.00000000000006e-05
12 -1.00000000000031e-05
13 1.99999999999992e-05
14 0.000110000000000006
15 0.000140000000000001
16 6.99999999999997e-05
17 -0.000109999999999999
18 -0.000270000000000006
19 -0.000200000000000006
20 -7.00000000000006e-05
21 2.99999999999988e-05
22 5.00000000000014e-05
23 3.99999999999845e-05
24 -9.9999999999989e-05
25 -0.000209999999999998
26 -7.99999999999967e-05
27 2.99999999999996e-05
28 -4.99999999999945e-05
29 -0.000150000000000004
30 -1.99999999999922e-05
31 -4.99999999999945e-05
32 -7.00000000000145e-05
33 -7.00000000000006e-05
34 -0.000100000000000003
35 -7.99999999999967e-05
36 0.000119999999999995
37 -7.00000000000145e-05
38 -7.99999999999967e-05
39 -8.9999999999979e-05
40 -8.00000000000245e-05
41 2.000000000002e-05
42 -8.00000000000245e-05
43 -7.99999999999967e-05
44 -9.00000000000067e-05
45 -7.99999999999967e-05
46 -7.99999999999967e-05
47 -7.00000000000145e-05
48 -6.99999999999867e-05
49 -6.99999999999867e-05
50 0
51 5.99999999999767e-05
52 -7.99999999999967e-05
53 -7.00000000000145e-05
54 -7.99999999999967e-05
55 0
56 -7.99999999999967e-05
57 -7.99999999999967e-05
58 -0.000290000000000012
59 -9.00000000000067e-05
60 -7.99999999999967e-05
61 -9.00000000000067e-05
62 -7.99999999999967e-05
63 -7.99999999999967e-05
64 -7.00000000000145e-05
65 -7.99999999999967e-05
66 -8.00000000000245e-05
67 -7.00000000000145e-05
68 -6.99999999999867e-05
69 -9.00000000000067e-05
70 3.00000000000022e-05
71 6.00000000000045e-05
72 -7.00000000000145e-05
73 -7.99999999999967e-05
74 5.99999999999767e-05
75 -8.00000000000245e-05
76 -6.99999999999867e-05
77 -7.00000000000145e-05
78 -7.00000000000145e-05
79 -7.00000000000145e-05
80 -7.00000000000145e-05
81 -7.99999999999967e-05
82 -6.99999999999867e-05
83 -2.000000000002e-05
84 -7.99999999999967e-05
85 -7.00000000000145e-05
86 -7.99999999999967e-05
87 -6.99999999999867e-05
88 -9.99999999999612e-06
89 -1.99999999999922e-05
90 -4.00000000000122e-05
91 -4.00000000000122e-05
92 -1.000000000001e-05
93 1.000000000001e-05
94 5.00000000000222e-05
95 7.99999999999967e-05
96 0.000190000000000023
97 0.000229999999999952
98 0.000299999999999967
99 0.000390000000000001
100 0.000390000000000001
101 0.000649999999999817
102 0.000580000000000025
103 0.00116000000000005
104 0.00129000000000001
105 0.00130000000000008
106 0.00140999999999991
107 0.00156000000000001
108 0.00165999999999977
109 0.00178000000000011
110 0.00193999999999983
111 0.00204000000000004
112 0.00220999999999982
113 0.00199999999999978
114 0.00190000000000001
115 0.00181000000000076
116 0.00178999999999974
117 0.00183999999999962
118 0.00180000000000025
119 0.00190000000000001
120 0.00192999999999977
121 0.00199000000000016
122 0.00201000000000029
123 0.00205000000000055
124 0.00209999999999955
125 0.00210000000000043
126 0.00213000000000019
127 0.00215000000000032
128 0.00224000000000046
129 0.00231999999999921
130 0.00229999999999997
131 0.00254999999999939
132 0.00261999999999851
133 0.0028800000000011
134 0.00300000000000011
135 0.00302000000000113
136 0.00286000000000008
137 0.00321999999999889
138 0.00330999999999904
139 0.00338999999999956
140 0.00343999999999944
141 0.00346999999999831
142 0.00348000000000148
143 0.00346000000000046
144 0.0034900000000011
145 0.00357999999999947
146 0.00361000000000011
147 0.00359999999999872
148 0.00356999999999985
149 0.00351000000000035
150 0.00340000000000096
151 0.0033000000000003
152 0.00324999999999953
153 0.00321999999999978
154 0.00309999999999988
155 0.0029899999999996
156 0.00290999999999997
157 0.00286000000000008
158 0.00279999999999969
159 0.00276999999999994
160 0.00280000000000058
161 0.00280000000000058
162 0.0028100000000002
163 0.00276999999999994
164 0.00276000000000032
165 0.00274000000000019
166 0.00281999999999982
167 0.00344000000000033
168 0.00325000000000042
169 0.00332000000000043
170 0.0034200000000002
171 0.00351999999999997
172 0.00358999999999909
173 0.00366
174 0.00374999999999837
175 0.00383999999999851
176 0.0039700000000007
177 0.00405999999999906
178 0.00411000000000072
179 0.00403999999999982
180 0.00384999999999991
181 0.00360000000000049
182 0.00337999999999994
183 0.00334000000000056
184 0.00335000000000019
185 0.00339000000000045
186 0.00344999999999995
187 0.00349999999999984
188 0.00356000000000023
189 0.00370999999999988
190 0.00381999999999927
191 0.00393000000000043
192 0.00400000000000134
193 0.0040400000000016
194 0.00402000000000058
195 0.00403999999999982
196 0.00403999999999982
197 0.00398000000000032
198 0.0039599999999993
199 0.00391999999999904
200 0.00380999999999965
201 0.00369000000000064
202 0.00355000000000061
203 0.0034200000000002
204 0.00328999999999979
205 0.00317000000000078
206 0.00305
207 0.00609000000000037
208 0.00309000000000026
209 0.00307000000000013
210 0.00297999999999998
211 0.0029300000000001
212 0.00283999999999995
213 0.00276999999999994
214 0.00274000000000019
215 0.00272000000000006
216 0.00265000000000004
217 0.00257000000000041
218 0.00248000000000026
219 0.00242999999999949
220 0.00236000000000036
221 0.00246999999999975
222 0.00263999999999953
223 0.00283000000000033
224 0.00296999999999947
225 0.00305
226 0.00306000000000051
227 0.00305
228 0.00305
229 0.00307000000000013
230 0.00307000000000013
231 0.00321000000000016
232 0.00323000000000029
233 0.00316000000000027
234 0.00309999999999988
235 0.00305
236 0.00294999999999934
237 0.00288000000000022
238 0.00284999999999958
239 0.00288000000000022
240 0.0029300000000001
241 0.00300000000000011
242 0.00307000000000013
243 0.00314000000000014
244 0.00321000000000016
245 0.00328999999999979
246 0.00341000000000058
247 0.00349999999999984
248 0.00362000000000062
249 0.00375999999999976
250 0.00390000000000068
251 0.00404999999999944
252 0.00421000000000049
253 0.00430000000000064
254 0.00439999999999952
255 0.00453000000000081
256 0.00465999999999944
257 0.00471999999999895
258 0.00466999999999906
259 0.00463000000000058
260 0.00445999999999991
261 0.00439999999999863
262 0.00428000000000139
263 0.00419000000000125
264 0.00405000000000122
265 0.00390999999999941
266 0.00378999999999863
267 0.00371000000000166
268 0.00363999999999898
269 0.00359000000000087
270 0.00358000000000125
271 0.00358000000000125
272 0.00355000000000061
273 0.00353999999999921
274 0.00348999999999933
275 0.00340999999999969
276 0.00328000000000017
277 0.00321000000000016
278 0.00314000000000014
279 0.00309000000000026
280 0.00307999999999975
281 0.0031800000000004
282 0.00319000000000003
283 0.00320000000000054
284 0.00321999999999978
285 0.00323000000000029
286 0.00319999999999965
287 0.00317999999999952
288 0.00314999999999976
289 0.00314000000000014
290 0.00313000000000052
291 0.00313000000000052
292 0.00312999999999963
293 0.00314999999999976
294 0.00314999999999976
295 0.00315000000000065
296 0.00303999999999949
297 0.00296999999999992
298 0.00290999999999997
299 0.00283999999999995
300 0.00275999999999987
301 0.00272000000000006
302 0.00273000000000012
303 0.00274000000000019
304 0.00272000000000006
305 0.00267000000000017
306 0.00260999999999978
307 0.00253000000000014
308 0.00245000000000006
309 0.00235000000000007
310 0.00229999999999997
311 0.00226000000000015
312 0.00219999999999998
313 0.00212000000000001
314 0.00205
315 0.00202999999999998
316 0.00204000000000004
317 0.00209000000000004
318 0.00214000000000003
319 0.00217000000000001
320 0.00221000000000005
321 0.00223000000000007
322 0.00226000000000004
323 0.00227999999999995
324 0.00229999999999997
325 0.00235000000000007
326 0.00239999999999996
327 0.00245000000000006
328 0.00252000000000008
329 0.00259000000000009
330 0.00262000000000007
331 0.00259999999999994
332 0.00255000000000005
333 0.00252999999999992
334 0.00244
335 0.00244
336 0.00244
337 0.00246000000000013
338 0.00248999999999988
339 0.00247000000000019
340 0.00244
341 0.00236999999999998
342 0.00234999999999985
343 0.00235999999999992
344 0.00236999999999998
345 0.00234999999999985
346 0.00229999999999997
347 0.00222999999999995
348 0.00213000000000019
349 0.00199000000000016
350 0.00184999999999991
351 0.0016799999999999
352 0.00153999999999999
353 0.00139
354 0.00121000000000002
355 0.00104000000000001
356 0.000919999999999976
357 0.00088000000000002
358 0.000879999999999992
359 0.000880000000000047
360 0.000860000000000027
361 0.000829999999999997
362 0.000800000000000023
363 0.000769999999999993
364 0.000769999999999993
365 0.000790000000000013
};
\addlegendentry{JPEG10}
\addplot [semithick, color1, mark=*, mark size=0.3, mark options={solid}, only marks]
table {%
0 0
1 0
2 0
3 0
4 0
5 0
6 0
7 0
8 -3.00000000000022e-05
9 -9.99999999999959e-06
10 -1.99999999999992e-05
11 -9.99999999999612e-06
12 1.00000000000031e-05
13 -9.99999999999959e-06
14 -1.99999999999992e-05
15 -1.99999999999992e-05
16 -8.99999999999998e-05
17 -2.99999999999953e-05
18 3.00000000000022e-05
19 2.99999999999884e-05
20 -2.00000000000061e-05
21 -5.00000000000014e-05
22 -3.99999999999984e-05
23 -7.00000000000145e-05
24 -9.9999999999989e-05
25 -7.99999999999985e-05
26 -6.00000000000045e-05
27 -7.00000000000006e-05
28 -7.99999999999967e-05
29 -8.99999999999998e-05
30 -5.99999999999906e-05
31 -4.99999999999945e-05
32 -6.00000000000045e-05
33 -9.00000000000067e-05
34 -0.000100000000000003
35 -7.99999999999967e-05
36 -8.99999999999929e-05
37 -9.00000000000067e-05
38 -0.000100000000000017
39 -0.000109999999999999
40 -0.000100000000000017
41 -9.99999999998225e-06
42 -0.000100000000000017
43 -9.9999999999989e-05
44 -0.000109999999999999
45 -8.9999999999979e-05
46 -5.99999999999767e-05
47 -9.00000000000067e-05
48 -9.9999999999989e-05
49 -9.00000000000067e-05
50 -9.00000000000067e-05
51 -2.000000000002e-05
52 -9.9999999999989e-05
53 0.000469999999999998
54 9.00000000000067e-05
55 -9.00000000000067e-05
56 -9.9999999999989e-05
57 -9.9999999999989e-05
58 -9.9999999999989e-05
59 -4.00000000000122e-05
60 -9.9999999999989e-05
61 -8.00000000000245e-05
62 -0.000100000000000017
63 -0.000109999999999999
64 -0.000100000000000017
65 -0.000109999999999999
66 -6.00000000000045e-05
67 -6.00000000000045e-05
68 -9.9999999999989e-05
69 -0.000109999999999999
70 -0.000109999999999999
71 -9.9999999999989e-05
72 -5.00000000000222e-05
73 -0.000109999999999999
74 -0.000100000000000017
75 -9.00000000000067e-05
76 -9.9999999999989e-05
77 -0.000100000000000017
78 -0.000100000000000017
79 -0.000100000000000017
80 -9.9999999999989e-05
81 -0.000109999999999999
82 -9.9999999999989e-05
83 -0.000100000000000017
84 -9.9999999999989e-05
85 -0.000100000000000017
86 -9.9999999999989e-05
87 -3.00000000000022e-05
88 0
89 0
90 -1.000000000001e-05
91 -3.00000000000022e-05
92 0
93 -9.99999999998225e-06
94 2.000000000002e-05
95 0
96 0
97 0
98 4.000000000004e-05
99 3.9999999999929e-05
100 -0.000130000000000075
101 -5.00000000001055e-05
102 0.000470000000000192
103 -0.000380000000000047
104 0.000390000000000112
105 0.00030999999999981
106 0.00030999999999981
107 0.000390000000000335
108 0.000420000000000087
109 0.000910000000000188
110 0.000779999999999781
111 0.000499999999999723
112 0.000329999999999941
113 0.000280000000000058
114 0.000140000000000029
115 0
116 7.00000000000145e-05
117 4.0000000000262e-05
118 -0.000719999999999388
119 -0.000230000000000175
120 -0.000300000000000189
121 -0.00032000000000032
122 -0.000340000000000451
123 -0.000319999999999432
124 -0.000390000000000335
125 -0.000409999999999577
126 -0.000460000000000349
127 -0.000499999999998835
128 -0.00046999999999997
129 -0.000560000000000116
130 -0.000729999999999009
131 -0.00081000000000131
132 -0.00109000000000137
133 -0.0015199999999993
134 -0.00154000000000032
135 -0.00155999999999956
136 -0.00157000000000096
137 -0.00154999999999994
138 -0.00154000000000032
139 -0.00150000000000006
140 -0.00143000000000093
141 -0.00136000000000003
142 -0.00131000000000014
143 -0.00112999999999985
144 -0.00103999999999971
145 -0.000950000000001339
146 -0.00100000000000122
147 -0.00101000000000084
148 -0.000939999999999941
149 -0.000890000000000057
150 -0.000849999999999795
151 -0.000799999999999912
152 -0.000770000000000159
153 -0.00075999999999965
154 -0.000770000000000159
155 -0.00063000000000013
156 -0.00046999999999997
157 -0.000560000000000116
158 -0.000570000000000626
159 -0.000550000000000495
160 -0.000539999999999985
161 -0.000529999999999475
162 -0.000389999999999446
163 -0.000560000000000116
164 -0.000680000000000014
165 -0.000680000000000014
166 -0.000680000000000014
167 -0.000649999999999373
168 -0.000700000000000145
169 -0.000820000000000043
170 -0.000859999999999417
171 -0.000930000000000319
172 -0.000989999999999824
173 -0.00102000000000046
174 -0.00105000000000111
175 -0.00106000000000073
176 -0.0011499999999991
177 -0.00118999999999936
178 -0.00131000000000014
179 -0.00126999999999988
180 -0.00124999999999886
181 -0.00122
182 -0.00103000000000009
183 -0.00100999999999996
184 -0.0010299999999992
185 -0.00103999999999971
186 -0.00112000000000023
187 -0.0011000000000001
188 -0.00112999999999985
189 -0.00112000000000023
190 -0.00116000000000049
191 -0.00121000000000038
192 -0.0012799999999995
193 -0.00132999999999939
194 -0.00132999999999939
195 -0.00134000000000079
196 -0.00134000000000079
197 -0.00134000000000079
198 -0.00136000000000003
199 -0.00136000000000003
200 -0.00137000000000143
201 -0.00136999999999965
202 -0.00133999999999901
203 -0.00136999999999965
204 -0.00133000000000116
205 -0.00131000000000014
206 -0.0012799999999995
207 -0.00118999999999936
208 -0.00113999999999947
209 -0.00117000000000012
210 -0.00117000000000012
211 -0.00121000000000038
212 -0.00114000000000036
213 -0.00110999999999972
214 -0.00112000000000023
215 -0.00112999999999985
216 -0.00109999999999921
217 -0.00103999999999971
218 -0.00104999999999933
219 -0.00107999999999997
220 -0.00110999999999972
221 -0.00112000000000023
222 -0.00111000000000061
223 -0.00108999999999959
224 -0.00105999999999984
225 -0.0010400000000006
226 -0.00103999999999971
227 -0.00105999999999984
228 -0.00107000000000035
229 -0.0011000000000001
230 -0.00114000000000036
231 -0.000989999999999824
232 -0.000999999999999446
233 -0.00103000000000009
234 -0.00102000000000046
235 -0.000989999999999824
236 -0.000960000000000072
237 -0.000949999999999562
238 -0.00095000000000045
239 -0.000939999999999941
240 -0.000939999999999941
241 -0.000930000000000319
242 -0.0009099999999993
243 -0.000890000000000057
244 -0.000879999999999548
245 -0.000890000000000057
246 -0.000859999999999417
247 -0.000849999999999795
248 -0.000829999999999664
249 -0.000849999999999795
250 -0.000829999999999664
251 -0.000850000000000684
252 -0.000899999999999679
253 -0.000869999999999926
254 -0.000900000000000567
255 -0.000989999999999824
256 -0.00102000000000046
257 -0.00106000000000073
258 -0.00112999999999985
259 -0.00109999999999921
260 -0.0012900000000009
261 -0.00139000000000067
262 -0.00145999999999979
263 -0.00136999999999965
264 -0.00137999999999927
265 -0.00140000000000029
266 -0.00139000000000067
267 -0.00138999999999889
268 -0.00131000000000014
269 -0.00133999999999901
270 -0.00134999999999863
271 -0.00132999999999939
272 -0.0012900000000009
273 -0.00125000000000064
274 -0.00123000000000051
275 -0.00129999999999963
276 -0.00117999999999974
277 -0.00114999999999998
278 -0.00109000000000048
279 -0.00103999999999971
280 -0.00100999999999996
281 -0.00105000000000022
282 -0.00103999999999971
283 -0.00101999999999958
284 -0.00102000000000046
285 -0.000960000000000072
286 -0.000970000000000582
287 -0.000930000000000319
288 -0.000930000000000319
289 -0.00091999999999981
290 -0.000929999999999431
291 -0.000929999999999431
292 -0.000930000000000319
293 -0.000930000000000319
294 -0.00091999999999981
295 -0.000829999999999664
296 -0.000860000000000305
297 -0.000820000000000043
298 -0.000809999999999977
299 -0.00079000000000029
300 -0.000750000000000028
301 -0.000760000000000094
302 -0.000750000000000028
303 -0.00075999999999965
304 -0.00075999999999965
305 -0.000750000000000028
306 -0.000729999999999897
307 -0.000729999999999897
308 -0.000649999999999817
309 -0.000659999999999883
310 -0.000680000000000014
311 -0.000669999999999948
312 -0.000650000000000039
313 -0.000669999999999948
314 -0.000649999999999928
315 -0.000630000000000019
316 -0.000650000000000039
317 -0.000650000000000039
318 -0.000649999999999928
319 -0.000650000000000039
320 -0.000649999999999928
321 -0.000649999999999928
322 -0.000639999999999974
323 -0.000630000000000019
324 -0.000640000000000085
325 -0.000629999999999908
326 -0.000640000000000196
327 -0.000629999999999908
328 -0.000650000000000039
329 -0.000650000000000039
330 -0.000649999999999817
331 -0.000660000000000105
332 -0.000669999999999948
333 -0.000680000000000014
334 -0.000739999999999963
335 -0.000709999999999766
336 -0.00071000000000021
337 -0.000699999999999701
338 -0.000700000000000145
339 -0.000709999999999766
340 -0.000739999999999963
341 -0.00071000000000021
342 -0.00071000000000021
343 -0.000709999999999766
344 -0.00071000000000021
345 -0.00071000000000021
346 -0.000719999999999832
347 -0.000730000000000119
348 -0.000739999999999963
349 -0.000750000000000028
350 -0.000750000000000028
351 -0.000739999999999963
352 -0.000750000000000028
353 -0.000740000000000018
354 -0.00083999999999998
355 -0.000799999999999995
356 -0.000810000000000005
357 -0.000819999999999987
358 -0.000820000000000043
359 -0.000789999999999957
360 -0.000800000000000023
361 -0.000800000000000023
362 -0.000800000000000023
363 -0.000800000000000023
364 -0.000809999999999977
365 -0.000840000000000007
};
\addlegendentry{JPEG50}
\end{axis}

\end{tikzpicture}

==> fig/yplot.tex <==
% This file was created by matplotlib2tikz v0.7.3.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.980392156862745,0.501960784313725,0.447058823529412}
\definecolor{color1}{rgb}{0.698039215686274,0.133333333333333,0.133333333333333}

\begin{axis}[
height=\figureheight,
legend cell align={left},
legend style={draw=white!80.0!black},
tick align=outside,
tick pos=left,
width=\figurewidth,
x grid style={white!69.01960784313725!black},
xmin=-18.25, xmax=383.25,
xtick style={color=black},
xtick={0,100,200,300},
xticklabels={0,50,100,150},
y grid style={white!69.01960784313725!black},
ymin=-0.000774500000000014, ymax=0.00526450000000029,
ytick style={color=black}
]
\addplot [semithick, color0, mark=*, mark size=0.3, mark options={solid}, only marks]
table {%
0 0
1 8.99999999999998e-05
2 8e-05
3 -2.99999999999988e-05
4 -5.00000000000001e-05
5 -0.000109999999999999
6 1.99999999999992e-05
7 4.00000000000001e-05
8 -8.00000000000002e-05
9 -1.00000000000013e-05
10 -3.00000000000022e-05
11 -6.99999999999989e-05
12 -2.99999999999953e-05
13 1.99999999999922e-05
14 0.000300000000000022
15 0.000470000000000026
16 0.000209999999999988
17 1.00000000000031e-05
18 -0.000140000000000001
19 -7.99999999999967e-05
20 4.00000000000018e-05
21 9.9999999999989e-05
22 0.000109999999999999
23 0.000190000000000023
24 0.000200000000000001
25 8.9999999999979e-05
26 0
27 0.000159999999999993
28 0.000200000000000006
29 0.000149999999999997
30 7.99999999999967e-05
31 -1.99999999999922e-05
32 9.99999999999959e-06
33 0.00018
34 0.000140000000000001
35 9e-05
36 0.00017
37 0.000189999999999999
38 0.00018
39 0.000189999999999999
40 0.000189999999999999
41 0.000190000000000003
42 0.00018
43 0.000189999999999999
44 0.000189999999999999
45 0.000189999999999999
46 0.000180000000000003
47 0.000189999999999999
48 0.00018
49 0.000189999999999999
50 0.000189999999999999
51 6.0000000000001e-05
52 0.000189999999999999
53 0.000189999999999999
54 0.000190000000000003
55 0.000189999999999999
56 0.000189999999999999
57 0.000190000000000003
58 -0.00026
59 5.00000000000014e-05
60 0.00016
61 0.000189999999999999
62 0.000189999999999999
63 0.00018
64 0.000180000000000003
65 0.000189999999999999
66 0.000189999999999999
67 0.00018
68 0.00018
69 0.000189999999999999
70 0.000189999999999999
71 0.000210000000000002
72 0.00018
73 0.000189999999999999
74 0.000199999999999999
75 0.000180000000000003
76 0.000189999999999999
77 0.000189999999999999
78 0.00018
79 0.000189999999999999
80 0.00018
81 0.000189999999999999
82 0.00018
83 0.000199999999999999
84 0.00018
85 0.00018
86 0.00018
87 0.00018
88 0.000159999999999993
89 0.000149999999999983
90 0.00018
91 0.000219999999999998
92 0.000199999999999978
93 0.000200000000000006
94 0.000180000000000013
95 0.000219999999999998
96 0.000199999999999978
97 0.000290000000000012
98 0.000360000000000027
99 0.000480000000000036
100 0.000609999999999999
101 0.000760000000000094
102 0.000859999999999861
103 0.000560000000000116
104 0.000990000000000046
105 0.00100999999999996
106 0.00114999999999998
107 0.00133000000000005
108 0.00146000000000002
109 0.00164000000000009
110 0.00181999999999993
111 0.00199999999999978
112 0.00211000000000006
113 0.00214000000000025
114 0.00233999999999979
115 0.00251999999999963
116 0.00265000000000004
117 0.00279999999999969
118 0.00296999999999992
119 0.00312000000000001
120 0.00321999999999978
121 0.00334000000000012
122 0.00341000000000014
123 0.00344999999999995
124 0.00347000000000008
125 0.00352999999999959
126 0.00362000000000018
127 0.00376000000000021
128 0.00389000000000017
129 0.00404999999999989
130 0.00422999999999973
131 0.00444999999999984
132 0.0046400000000002
133 0.00483000000000011
134 0.00499000000000027
135 0.00488999999999962
136 0.00484000000000062
137 0.00490000000000013
138 0.00488999999999962
139 0.00483999999999973
140 0.00476999999999972
141 0.00469000000000008
142 0.00459000000000032
143 0.00443000000000016
144 0.00429000000000013
145 0.00416999999999934
146 0.00405999999999995
147 0.00394999999999968
148 0.00385999999999953
149 0.00377000000000027
150 0.00366999999999962
151 0.0035400000000001
152 0.00339999999999918
153 0.00326999999999966
154 0.0031099999999995
155 0.00290999999999997
156 0.00276000000000032
157 0.00262999999999991
158 0.00255000000000027
159 0.00249999999999995
160 0.00250000000000039
161 0.00256999999999952
162 0.00265999999999966
163 0.00273000000000012
164 0.00279999999999969
165 0.00281999999999982
166 0.00283000000000033
167 0.00334000000000056
168 0.00314000000000014
169 0.00322000000000067
170 0.00338999999999956
171 0.00354999999999972
172 0.00366
173 0.00375999999999976
174 0.00386000000000042
175 0.00392999999999954
176 0.00402000000000058
177 0.00417000000000023
178 0.00434000000000001
179 0.00441000000000003
180 0.00427999999999962
181 0.00389999999999979
182 0.00353000000000048
183 0.00332000000000043
184 0.00321000000000016
185 0.00319999999999965
186 0.00328000000000017
187 0.00340999999999969
188 0.00352999999999959
189 0.00368000000000013
190 0.00389999999999979
191 0.00408000000000008
192 0.00429999999999975
193 0.00450000000000017
194 0.00464999999999982
195 0.0047600000000001
196 0.00485000000000024
197 0.00490999999999975
198 0.00493000000000077
199 0.00485999999999986
200 0.00471000000000021
201 0.00459000000000032
202 0.00445000000000029
203 0.00431000000000026
204 0.0041500000000001
205 0.00396999999999981
206 0.00380000000000003
207 0.00227000000000022
208 0.0033499999999993
209 0.00314000000000014
210 0.00295000000000023
211 0.00276999999999994
212 0.00260999999999978
213 0.00247000000000019
214 0.00234000000000023
215 0.00221999999999989
216 0.00208999999999993
217 0.0019499999999999
218 0.00188999999999995
219 0.00193000000000021
220 0.00202999999999998
221 0.00214999999999987
222 0.00224000000000002
223 0.0022899999999999
224 0.00231000000000003
225 0.0023200000000001
226 0.00239000000000011
227 0.00245000000000006
228 0.00251000000000001
229 0.00256999999999996
230 0.00265000000000004
231 0.00267000000000017
232 0.00268999999999986
233 0.00260999999999978
234 0.00251000000000001
235 0.00241000000000025
236 0.00233000000000017
237 0.00225999999999971
238 0.00221999999999989
239 0.0022000000000002
240 0.00215000000000032
241 0.00213000000000019
242 0.00209999999999999
243 0.00207999999999986
244 0.00209999999999955
245 0.00215000000000032
246 0.00215999999999994
247 0.00218000000000007
248 0.00225000000000009
249 0.0023799999999996
250 0.00257000000000041
251 0.00272000000000006
252 0.00288000000000022
253 0.00311000000000039
254 0.00333999999999968
255 0.0035400000000001
256 0.00370999999999988
257 0.00385999999999953
258 0.00363000000000024
259 0.00410999999999984
260 0.00436999999999976
261 0.00450000000000017
262 0.00455000000000005
263 0.00451999999999941
264 0.00445999999999991
265 0.00431999999999988
266 0.00419999999999998
267 0.00404999999999944
268 0.00394999999999968
269 0.00388000000000055
270 0.00382000000000016
271 0.00372000000000039
272 0.00360999999999922
273 0.00347999999999971
274 0.00333999999999968
275 0.0031800000000004
276 0.00307999999999975
277 0.00295999999999985
278 0.00282999999999944
279 0.00272000000000006
280 0.00264000000000042
281 0.00251999999999963
282 0.00246999999999975
283 0.0023799999999996
284 0.00228000000000073
285 0.00218999999999969
286 0.00211000000000006
287 0.00201000000000029
288 0.00194000000000027
289 0.00189000000000039
290 0.00185000000000013
291 0.00180999999999987
292 0.00175999999999998
293 0.00168999999999997
294 0.00164000000000009
295 0.00147999999999993
296 0.00140999999999991
297 0.00129999999999963
298 0.00117000000000012
299 0.00104999999999977
300 0.000969999999999693
301 0.000939999999999941
302 0.000909999999999744
303 0.000859999999999861
304 0.000780000000000225
305 0.000640000000000196
306 0.000510000000000232
307 0.000379999999999825
308 0.000259999999999927
309 0.000159999999999716
310 0.000110000000000277
311 7.00000000000145e-05
312 1.00000000000655e-05
313 -7.00000000000145e-05
314 -0.000119999999999898
315 -0.000129999999999963
316 -9.00000000001455e-05
317 -8.000000000008e-05
318 -5.9999999999949e-05
319 -5.00000000003276e-05
320 -5.9999999999949e-05
321 -9.00000000001455e-05
322 -9.99999999997669e-05
323 -9.00000000001455e-05
324 -5.9999999999949e-05
325 -2.99999999997524e-05
326 7.00000000000145e-05
327 0.00016000000000016
328 0.000199999999999978
329 0.00022999999999973
330 0.000249999999999861
331 0.000260000000000371
332 0.000279999999999614
333 0.000340000000000007
334 0.000420000000000087
335 0.00046999999999997
336 0.000520000000000298
337 0.000539999999999985
338 0.00055000000000005
339 0.000529999999999919
340 0.000490000000000101
341 0.000449999999999839
342 0.000429999999999708
343 0.000449999999999839
344 0.000459999999999905
345 0.000460000000000349
346 0.000440000000000218
347 0.000410000000000021
348 0.000329999999999941
349 0.000299999999999967
350 0.000180000000000069
351 0.000110000000000054
352 1.00000000000655e-05
353 -0.000120000000000009
354 -0.000249999999999972
355 -0.000340000000000007
356 -0.000380000000000005
357 -0.000400000000000005
358 -0.000420000000000004
359 -0.000459999999999999
360 -0.000480000000000001
361 -0.000490000000000004
362 -0.00048999999999999
363 -0.000480000000000008
364 -0.00048999999999999
365 -0.0005
};
\addlegendentry{JPEG10}
\addplot [semithick, color1, mark=*, mark size=0.3, mark options={solid}, only marks]
table {%
0 0
1 0
2 0
3 0
4 0
5 0
6 0
7 0
8 -2.99999999999996e-05
9 -1.00000000000013e-05
10 -1.00000000000031e-05
11 -2.99999999999988e-05
12 -2.99999999999953e-05
13 0
14 3.99999999999845e-05
15 2.99999999999745e-05
16 0.000159999999999993
17 0.000129999999999998
18 6.00000000000045e-05
19 6.00000000000045e-05
20 0.000100000000000003
21 0.000139999999999973
22 0.000129999999999991
23 0.000120000000000009
24 9.00000000000007e-05
25 4.99999999999945e-05
26 8.00000000000002e-05
27 0.000139999999999973
28 0.000140000000000001
29 0.000119999999999995
30 0.000109999999999999
31 7.99999999999967e-05
32 8.99999999999998e-05
33 0.000109999999999999
34 8.99999999999998e-05
35 0.0001
36 0.000110000000000002
37 9.99999999999994e-05
38 9.99999999999994e-05
39 9.99999999999994e-05
40 9.99999999999994e-05
41 0.000110000000000002
42 0.000109999999999999
43 0.000109999999999999
44 0.000109999999999999
45 0.000109999999999999
46 0.000110000000000002
47 0.000109999999999999
48 9.99999999999994e-05
49 0.000110000000000002
50 9.99999999999994e-05
51 0.000110000000000002
52 0.000109999999999999
53 0
54 0.000130000000000002
55 9.99999999999994e-05
56 0.000109999999999999
57 0.000110000000000002
58 9.99999999999994e-05
59 0.000100000000000003
60 9.99999999999994e-05
61 0.000109999999999999
62 9.99999999999994e-05
63 9.99999999999994e-05
64 0.000100000000000003
65 9.99999999999994e-05
66 0.000109999999999999
67 0.000109999999999999
68 9.99999999999994e-05
69 0.000109999999999999
70 9.99999999999994e-05
71 0.000109999999999999
72 0.000109999999999999
73 0.000109999999999999
74 9.99999999999994e-05
75 0.000110000000000002
76 0.000109999999999999
77 0.000109999999999999
78 0.000110000000000002
79 0.000109999999999999
80 9.99999999999994e-05
81 0.000109999999999999
82 9.99999999999994e-05
83 0.000109999999999999
84 9.99999999999994e-05
85 9.99999999999994e-05
86 0.000100000000000003
87 0.000100000000000003
88 0.000130000000000005
89 0.000120000000000009
90 0.000130000000000005
91 0.000119999999999995
92 9.9999999999989e-05
93 0.000109999999999999
94 0.000159999999999993
95 0.000159999999999993
96 0.000199999999999978
97 0.000260000000000038
98 0.000280000000000058
99 0.000330000000000052
100 0.000369999999999981
101 0.000460000000000127
102 0.000589999999999868
103 0.000530000000000141
104 0.000420000000000087
105 0.000439999999999996
106 0.000450000000000061
107 0.000490000000000101
108 0.000520000000000076
109 0.000439999999999996
110 0.000499999999999945
111 0.000569999999999737
112 0.000510000000000232
113 0.000530000000000364
114 0.000599999999999934
115 0.000680000000000014
116 0.000640000000000196
117 0.000669999999999948
118 0.000669999999999948
119 0.000690000000000079
120 0.000699999999999701
121 0.000760000000000094
122 0.000760000000000094
123 0.000779999999999781
124 0.000820000000000043
125 0.000849999999999795
126 0.000879999999999992
127 0.000950000000000006
128 0.00102000000000002
129 0.00105000000000022
130 0.00111999999999979
131 0.00116999999999967
132 0.00127999999999995
133 0.00144000000000011
134 0.00163000000000046
135 0.00166999999999984
136 0.00181000000000076
137 0.00189000000000039
138 0.00194000000000027
139 0.00195999999999952
140 0.00197999999999965
141 0.00197000000000003
142 0.00195000000000078
143 0.00192999999999977
144 0.00189000000000039
145 0.0018899999999995
146 0.00187999999999988
147 0.00175999999999998
148 0.00176999999999961
149 0.00173000000000023
150 0.00180000000000025
151 0.00154000000000032
152 0.00149999999999917
153 0.00144999999999929
154 0.00138000000000016
155 0.00122
156 0.00108999999999959
157 0.00110999999999972
158 0.00109000000000004
159 0.0010699999999999
160 0.00106000000000028
161 0.00108999999999959
162 0.00105000000000022
163 0.0011000000000001
164 0.00110999999999972
165 0.00111000000000017
166 0.00112000000000023
167 0.00119999999999987
168 0.00145000000000017
169 0.00154000000000032
170 0.00161999999999995
171 0.00168999999999997
172 0.00174999999999947
173 0.00181999999999949
174 0.00187000000000026
175 0.00192999999999977
176 0.00201999999999991
177 0.00216999999999956
178 0.00230999999999959
179 0.00227000000000022
180 0.00218999999999969
181 0.00201999999999991
182 0.00180999999999987
183 0.00174000000000074
184 0.0017100000000001
185 0.00173999999999985
186 0.00175999999999998
187 0.00177999999999923
188 0.00181999999999949
189 0.00186000000000064
190 0.0019499999999999
191 0.00202999999999953
192 0.00209999999999955
193 0.00214999999999943
194 0.00218000000000007
195 0.00220999999999982
196 0.00222000000000033
197 0.00221999999999944
198 0.00222000000000033
199 0.00218000000000007
200 0.00215999999999994
201 0.00211999999999968
202 0.00204000000000004
203 0.00199000000000016
204 0.00191000000000052
205 0.00182000000000038
206 0.00175999999999998
207 0.00167999999999946
208 0.00160999999999945
209 0.00158000000000014
210 0.00155000000000038
211 0.00151999999999974
212 0.00146999999999986
213 0.00143000000000004
214 0.00138000000000016
215 0.00135999999999958
216 0.00131999999999977
217 0.00125999999999982
218 0.00122
219 0.00122
220 0.00120999999999993
221 0.00123999999999969
222 0.00129000000000001
223 0.00136000000000003
224 0.00139999999999985
225 0.00139000000000022
226 0.00139999999999985
227 0.00141999999999998
228 0.00143999999999966
229 0.00145999999999979
230 0.00150000000000006
231 0.00148999999999999
232 0.00150000000000006
233 0.00145999999999979
234 0.00141999999999998
235 0.00138000000000016
236 0.00132999999999983
237 0.00129000000000001
238 0.00126000000000026
239 0.00129000000000001
240 0.00127000000000033
241 0.00127999999999995
242 0.00130000000000008
243 0.00132000000000021
244 0.00132999999999939
245 0.0013399999999999
246 0.0013399999999999
247 0.00137000000000054
248 0.00140000000000029
249 0.00147999999999993
250 0.00150999999999968
251 0.00157000000000007
252 0.00164999999999971
253 0.00167000000000073
254 0.00173999999999985
255 0.00186000000000064
256 0.00193999999999939
257 0.00198999999999927
258 0.0015900000000002
259 0.00187999999999988
260 0.00201000000000029
261 0.00201999999999991
262 0.00200000000000067
263 0.00202999999999953
264 0.00199000000000016
265 0.0019499999999999
266 0.0018899999999995
267 0.00183999999999962
268 0.00175999999999998
269 0.00177000000000049
270 0.00174999999999947
271 0.00173000000000023
272 0.00169999999999959
273 0.00167999999999946
274 0.00166000000000022
275 0.00163000000000046
276 0.00152999999999981
277 0.00147999999999993
278 0.00143000000000004
279 0.00138999999999978
280 0.00138000000000016
281 0.00136999999999965
282 0.00138000000000016
283 0.00136999999999965
284 0.0013399999999999
285 0.00131999999999977
286 0.00129999999999963
287 0.00128000000000039
288 0.00126000000000026
289 0.00124999999999975
290 0.00124999999999975
291 0.00124999999999975
292 0.00125000000000064
293 0.00123999999999924
294 0.00122999999999962
295 0.00117000000000012
296 0.00117000000000012
297 0.00112999999999985
298 0.0011000000000001
299 0.00105999999999984
300 0.00102999999999964
301 0.00100999999999996
302 0.00099999999999989
303 0.00100999999999996
304 0.000990000000000268
305 0.000960000000000072
306 0.000929999999999875
307 0.000889999999999613
308 0.000830000000000108
309 0.000769999999999715
310 0.000760000000000094
311 0.000779999999999781
312 0.000739999999999963
313 0.000719999999999832
314 0.000690000000000079
315 0.000659999999999883
316 0.000700000000000145
317 0.00071000000000021
318 0.000709999999999766
319 0.000719999999999832
320 0.000719999999999832
321 0.000719999999999832
322 0.000720000000000276
323 0.000729999999999897
324 0.000750000000000028
325 0.000750000000000028
326 0.000779999999999781
327 0.000779999999999781
328 0.000809999999999977
329 0.000819999999999599
330 0.000830000000000108
331 0.000840000000000174
332 0.00083999999999973
333 0.00083999999999973
334 0.000859999999999861
335 0.000859999999999861
336 0.00087000000000037
337 0.000869999999999926
338 0.000869999999999926
339 0.000869999999999926
340 0.000909999999999744
341 0.000869999999999926
342 0.000849999999999795
343 0.000849999999999795
344 0.000840000000000174
345 0.000840000000000174
346 0.000840000000000174
347 0.000829999999999664
348 0.000799999999999912
349 0.000790000000000068
350 0.000750000000000028
351 0.000690000000000079
352 0.000680000000000014
353 0.000639999999999974
354 0.000670000000000059
355 0.000630000000000019
356 0.000600000000000003
357 0.000599999999999996
358 0.000599999999999996
359 0.000580000000000001
360 0.00059
361 0.000579999999999997
362 0.000570000000000015
363 0.000579999999999997
364 0.000570000000000015
365 0.000570000000000015
};
\addlegendentry{JPEG50}
\end{axis}

\end{tikzpicture}

==> fig/zplot.tex <==
% This file was created by matplotlib2tikz v0.7.3.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.980392156862745,0.501960784313725,0.447058823529412}
\definecolor{color1}{rgb}{0.698039215686274,0.133333333333333,0.133333333333333}

\begin{axis}[
height=\figureheight,
legend cell align={left},
legend style={draw=white!80.0!black},
tick align=outside,
tick pos=left,
width=\figurewidth,
x grid style={white!69.01960784313725!black},
xmin=-18.25, xmax=383.25,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ymin=-0.00119950000000003, ymax=0.0049495,
ytick style={color=black}
]
\addplot [semithick, color0, mark=*, mark size=0.3, mark options={solid}, only marks]
table {%
0 0
1 1.000000000001e-05
2 0.00467
3 0.00146
4 0.00136999999999998
5 0.00143
6 0.00145999999999999
7 0.00140999999999998
8 0.00142000000000003
9 0.00143
10 0.00144
11 0.00144000000000001
12 0.00140999999999999
13 0.0014
14 0.00137999999999999
15 0.00135
16 0.00137999999999999
17 0.00146
18 0.00153
19 0.00147
20 0.00144
21 0.00142
22 0.00142
23 0.00143
24 0.00145
25 0.00144
26 0.00144
27 0.00146
28 0.00146
29 0.00145
30 0.00145
31 0.00146
32 0.00145
33 0.00145
34 0.00144
35 0.00145
36 0.00164
37 0.00144
38 0.00142999999999999
39 0.00144
40 0.00143000000000001
41 0.00145000000000001
42 0.00144
43 0.00142999999999999
44 0.00144
45 0.00142999999999999
46 0.00144
47 0.00143000000000001
48 0.00143000000000001
49 0.00143000000000001
50 0.00143000000000001
51 0.0018
52 0.00142999999999999
53 0.00142999999999999
54 0.00142999999999999
55 0.00142999999999999
56 0.00142999999999999
57 0.00143000000000001
58 0.00161
59 0.00144
60 0.00143000000000001
61 0.00142999999999999
62 0.00142999999999999
63 0.00144
64 0.00143000000000001
65 0.00142999999999999
66 0.00144
67 0.00143000000000001
68 0.00142999999999999
69 0.00144
70 0.00146000000000002
71 0.00147
72 0.00142999999999999
73 0.00144
74 0.00145999999999999
75 0.00144
76 0.00144
77 0.00144
78 0.00143000000000001
79 0.00144
80 0.00144
81 0.00142999999999999
82 0.00144
83 0.00144
84 0.00144
85 0.00143000000000001
86 0.00143000000000001
87 0.00142999999999999
88 0.00142999999999999
89 0.00145000000000001
90 0.00144
91 0.00145000000000001
92 0.00144999999999999
93 0.00144
94 0.00145000000000001
95 0.00144
96 0.00146000000000002
97 0.00144
98 0.00145000000000001
99 0.00145000000000001
100 0.00146999999999997
101 0.00142
102 0.00147999999999998
103 0.00151999999999999
104 0.00126
105 0.0013
106 0.00131
107 0.0013
108 0.00133
109 0.00131
110 0.00133
111 0.00140000000000001
112 0.00141999999999998
113 0.00118000000000001
114 0.00123000000000001
115 0.00121000000000004
116 0.00120999999999999
117 0.00120999999999999
118 0.00120000000000001
119 0.00120000000000001
120 0.00120000000000001
121 0.00115
122 0.00120000000000001
123 0.00119
124 0.00116999999999999
125 0.00120000000000001
126 0.00122
127 0.00120999999999999
128 0.00121
129 0.00121
130 0.00135000000000002
131 0.00124
132 0.00124
133 0.00115000000000001
134 0.00119999999999999
135 0.00122999999999999
136 0.00128
137 0.00125
138 0.00125000000000003
139 0.00126000000000004
140 0.00124999999999997
141 0.00126000000000004
142 0.00125999999999998
143 0.00125999999999998
144 0.00126000000000001
145 0.00125999999999998
146 0.00126999999999999
147 0.00126999999999999
148 0.00126999999999999
149 0.00127000000000002
150 0.00127000000000001
151 0.00126999999999999
152 0.00126999999999999
153 0.00128
154 0.00127
155 0.00128
156 0.00128
157 0.00128
158 0.00128
159 0.00129000000000001
160 0.00129999999999997
161 0.00127999999999995
162 0.00126999999999999
163 0.00125999999999993
164 0.00123999999999991
165 0.00126000000000004
166 0.0012500000000002
167 0.00157000000000007
168 0.00130999999999992
169 0.00126000000000004
170 0.00129000000000001
171 0.00126999999999988
172 0.00125999999999982
173 0.00126000000000004
174 0.00126999999999988
175 0.00126999999999988
176 0.0012700000000001
177 0.0012700000000001
178 0.00126000000000004
179 0.00126000000000004
180 0.0012700000000001
181 0.00125999999999982
182 0.00126999999999999
183 0.00126999999999999
184 0.00126999999999999
185 0.00126000000000004
186 0.00126999999999999
187 0.00126999999999999
188 0.0012700000000001
189 0.00126000000000004
190 0.0012700000000001
191 0.00125999999999982
192 0.00124999999999997
193 0.00124999999999997
194 0.00124999999999997
195 0.00126000000000004
196 0.00126000000000004
197 0.00126000000000004
198 0.0012700000000001
199 0.00127999999999995
200 0.00126000000000004
201 0.00125999999999982
202 0.00126000000000004
203 0.00126999999999988
204 0.00126000000000004
205 0.00126000000000004
206 0.00126000000000004
207 0.00143000000000004
208 0.00126999999999988
209 0.00124999999999997
210 0.00125999999999982
211 0.00126000000000004
212 0.00126000000000004
213 0.00125999999999982
214 0.00126000000000004
215 0.00126000000000004
216 0.00127999999999995
217 0.00126000000000004
218 0.00125999999999982
219 0.00126000000000004
220 0.00126000000000004
221 0.00125999999999982
222 0.00124999999999997
223 0.00124999999999997
224 0.00124999999999997
225 0.00126000000000004
226 0.00124999999999997
227 0.00124999999999997
228 0.00124999999999997
229 0.00124999999999997
230 0.00126999999999999
231 0.00134000000000001
232 0.00133000000000005
233 0.0012899999999999
234 0.00129000000000001
235 0.00129999999999997
236 0.00129000000000001
237 0.00131000000000003
238 0.00129999999999997
239 0.00131000000000003
240 0.00130999999999992
241 0.00130999999999992
242 0.00130000000000008
243 0.00130999999999992
244 0.00130999999999992
245 0.00131000000000014
246 0.00130999999999992
247 0.00131000000000014
248 0.00130999999999992
249 0.00130000000000008
250 0.00131000000000014
251 0.00131999999999999
252 0.00137999999999994
253 0.0013399999999999
254 0.00131999999999999
255 0.00131999999999999
256 0.00131999999999999
257 0.00131999999999999
258 0.000969999999999915
259 0.00136999999999987
260 0.00140000000000007
261 0.00137999999999994
262 0.00137999999999994
263 0.00134999999999996
264 0.00135000000000018
265 0.00134000000000012
266 0.00133000000000005
267 0.00133000000000005
268 0.00132999999999983
269 0.00131999999999999
270 0.00131999999999999
271 0.00131999999999999
272 0.00132999999999983
273 0.00131999999999999
274 0.00131999999999999
275 0.00133000000000005
276 0.00133000000000005
277 0.00131999999999999
278 0.00131999999999999
279 0.00131999999999999
280 0.00131999999999999
281 0.00130999999999992
282 0.00133000000000005
283 0.00131999999999999
284 0.00133000000000005
285 0.00131999999999999
286 0.00131999999999999
287 0.00131999999999999
288 0.00131999999999999
289 0.00131999999999999
290 0.00131999999999999
291 0.00131999999999999
292 0.00131999999999999
293 0.00131000000000003
294 0.0013200000000001
295 0.00129000000000001
296 0.00131999999999999
297 0.0013200000000001
298 0.00131999999999999
299 0.00132999999999994
300 0.00133
301 0.00132000000000004
302 0.00132999999999994
303 0.00131999999999999
304 0.00132999999999994
305 0.00131999999999999
306 0.00132000000000004
307 0.00129999999999997
308 0.00131000000000003
309 0.00133
310 0.00133
311 0.00132
312 0.0013
313 0.00131000000000001
314 0.00131
315 0.00131000000000001
316 0.0013
317 0.00130000000000001
318 0.00130999999999999
319 0.00130999999999998
320 0.00131000000000003
321 0.00131000000000003
322 0.00130999999999992
323 0.00129999999999997
324 0.00129999999999997
325 0.00130000000000008
326 0.00130000000000008
327 0.00129999999999986
328 0.00129000000000001
329 0.00131000000000014
330 0.00130000000000008
331 0.00130000000000008
332 0.00130000000000008
333 0.00129999999999986
334 0.00128000000000017
335 0.00128000000000017
336 0.0012700000000001
337 0.00126000000000004
338 0.00125999999999982
339 0.00126000000000004
340 0.00124999999999997
341 0.00124999999999997
342 0.00123999999999996
343 0.00123999999999999
344 0.00124
345 0.00124
346 0.00124
347 0.00124
348 0.00123999999999999
349 0.00117
350 0.00128
351 0.00127000000000002
352 0.00126999999999999
353 0.00127999999999998
354 0.00129000000000001
355 0.00129000000000001
356 0.00129000000000001
357 0.00128
358 0.00128
359 0.00128
360 0.00128
361 0.00128
362 0.00128
363 0.00128
364 0.00128
365 0.00128999999999999
};
\addlegendentry{JPEG10}
\addplot [semithick, color1, mark=*, mark size=0.3, mark options={solid}, only marks]
table {%
0 0
1 0
2 0
3 0
4 0
5 0
6 0
7 0
8 0
9 -9.99999999999612e-06
10 0
11 0
12 -1.000000000001e-05
13 -9.99999999999612e-06
14 9.99999999999612e-06
15 1.00000000000031e-05
16 4.99999999999945e-05
17 9.99999999999612e-06
18 -1.99999999999922e-05
19 -9.99999999999612e-06
20 2.99999999999884e-05
21 3.99999999999984e-05
22 3.00000000000022e-05
23 3.00000000000022e-05
24 2.99999999999988e-05
25 4.00000000000018e-05
26 4.00000000000001e-05
27 4.99999999999997e-05
28 5.00000000000001e-05
29 4.00000000000001e-05
30 5.00000000000014e-05
31 4.99999999999997e-05
32 4.00000000000001e-05
33 4.00000000000001e-05
34 4.00000000000001e-05
35 3.99999999999984e-05
36 3.00000000000022e-05
37 3.99999999999845e-05
38 1.99999999999922e-05
39 3.00000000000022e-05
40 3.00000000000022e-05
41 3.99999999999845e-05
42 3.00000000000022e-05
43 3.00000000000022e-05
44 3.00000000000022e-05
45 3.00000000000022e-05
46 3.00000000000022e-05
47 3.00000000000022e-05
48 3.00000000000022e-05
49 1.99999999999922e-05
50 3.00000000000022e-05
51 3.00000000000022e-05
52 1.99999999999922e-05
53 7.99999999999967e-05
54 3.99999999999845e-05
55 3.00000000000022e-05
56 3.00000000000022e-05
57 3.00000000000022e-05
58 2.000000000002e-05
59 3.00000000000022e-05
60 1.99999999999922e-05
61 3.00000000000022e-05
62 3.00000000000022e-05
63 3.00000000000022e-05
64 3.00000000000022e-05
65 1.99999999999922e-05
66 4.00000000000122e-05
67 3.00000000000022e-05
68 3.00000000000022e-05
69 3.00000000000022e-05
70 2.000000000002e-05
71 3.00000000000022e-05
72 3.00000000000022e-05
73 3.00000000000022e-05
74 3.00000000000022e-05
75 3.00000000000022e-05
76 3.00000000000022e-05
77 3.00000000000022e-05
78 3.00000000000022e-05
79 3.00000000000022e-05
80 3.00000000000022e-05
81 3.00000000000022e-05
82 3.00000000000022e-05
83 3.00000000000022e-05
84 3.00000000000022e-05
85 3.00000000000022e-05
86 2.000000000002e-05
87 4.99999999999945e-05
88 3.99999999999845e-05
89 4.00000000000122e-05
90 5.00000000000014e-05
91 3.00000000000022e-05
92 2.99999999999884e-05
93 3.00000000000022e-05
94 4.00000000000122e-05
95 2.99999999999745e-05
96 2.99999999999745e-05
97 1.99999999999645e-05
98 2.000000000002e-05
99 1.000000000001e-05
100 2.99999999999745e-05
101 0
102 -0.000230000000000008
103 0.000140000000000001
104 -0.000219999999999998
105 -0.000210000000000002
106 -0.00021
107 -0.000239999999999997
108 -0.00025
109 -0.000410000000000001
110 -0.000350000000000017
111 -0.000310000000000032
112 -0.000420000000000031
113 -0.00047999999999998
114 -0.000450000000000006
115 -0.00045999999999996
116 -0.0005
117 -0.00046999999999997
118 -0.00048999999999999
119 -0.000539999999999985
120 -0.000530000000000003
121 -0.000559999999999991
122 -0.000509999999999983
123 -0.000540000000000013
124 -0.000530000000000003
125 -0.000519999999999993
126 -0.00052000000000002
127 -0.000569999999999987
128 -0.000490000000000004
129 -0.000570000000000001
130 -0.000530000000000003
131 -0.000509999999999997
132 -0.000529999999999999
133 -0.000599999999999996
134 -0.000610000000000013
135 -0.000580000000000004
136 -0.000540000000000006
137 -0.000570000000000001
138 -0.000609999999999999
139 -0.000599999999999989
140 -0.000580000000000025
141 -0.000599999999999989
142 -0.000600000000000045
143 -0.000630000000000019
144 -0.000599999999999989
145 -0.000620000000000009
146 -0.000640000000000002
147 -0.000620000000000009
148 -0.000620000000000009
149 -0.000609999999999999
150 -0.000559999999999991
151 -0.000600000000000003
152 -0.000630000000000019
153 -0.000619999999999996
154 -0.000620000000000001
155 -0.0006
156 -0.000590000000000007
157 -0.000599999999999989
158 -0.000609999999999999
159 -0.000620000000000065
160 -0.000630000000000019
161 -0.000630000000000019
162 -0.000400000000000067
163 -0.000630000000000019
164 -0.000620000000000065
165 -0.000629999999999908
166 -0.000649999999999817
167 -0.000660000000000105
168 -0.000680000000000014
169 -0.000689999999999857
170 -0.000709999999999988
171 -0.000730000000000119
172 -0.000720000000000054
173 -0.000719999999999832
174 -0.000709999999999988
175 -0.000690000000000079
176 -0.000639999999999974
177 -0.000669999999999948
178 -0.000650000000000039
179 -0.000680000000000014
180 -0.000669999999999948
181 -0.000660000000000105
182 -0.000659999999999994
183 -0.000680000000000014
184 -0.000680000000000014
185 -0.000669999999999948
186 -0.000630000000000019
187 -0.000630000000000019
188 -0.000629999999999908
189 -0.000639999999999974
190 -0.000649999999999817
191 -0.000639999999999974
192 -0.00063000000000013
193 -0.000629999999999908
194 -0.000639999999999974
195 -0.000650000000000039
196 -0.000639999999999974
197 -0.000639999999999974
198 -0.000639999999999974
199 -0.00063000000000013
200 -0.000639999999999974
201 -0.00063000000000013
202 -0.000620000000000065
203 -0.000620000000000065
204 -0.000629999999999908
205 -0.000639999999999974
206 -0.000629999999999908
207 -0.000629999999999908
208 -0.000629999999999908
209 -0.000639999999999974
210 -0.00063000000000013
211 -0.000629999999999908
212 -0.00063000000000013
213 -0.000650000000000039
214 -0.000629999999999908
215 -0.000620000000000065
216 -0.000620000000000065
217 -0.000620000000000065
218 -0.00063000000000013
219 -0.00063000000000013
220 -0.000620000000000065
221 -0.000620000000000065
222 -0.000609999999999999
223 -0.000619999999999954
224 -0.000620000000000065
225 -0.000609999999999999
226 -0.000609999999999999
227 -0.000609999999999999
228 -0.000609999999999999
229 -0.000600000000000045
230 -0.000580000000000025
231 -0.000499999999999945
232 -0.00051000000000001
233 -0.000560000000000005
234 -0.000560000000000005
235 -0.000560000000000005
236 -0.00055000000000005
237 -0.000549999999999939
238 -0.000560000000000005
239 -0.000529999999999919
240 -0.000560000000000005
241 -0.00055000000000005
242 -0.000560000000000005
243 -0.00055000000000005
244 -0.00055000000000005
245 -0.000549999999999828
246 -0.000560000000000116
247 -0.00055000000000005
248 -0.000560000000000116
249 -0.000580000000000025
250 -0.000580000000000025
251 -0.000580000000000025
252 -0.000580000000000025
253 -0.00059000000000009
254 -0.00059000000000009
255 -0.000580000000000025
256 -0.000569999999999959
257 -0.000569999999999959
258 -0.000920000000000032
259 -0.000529999999999919
260 -0.000499999999999945
261 -0.000499999999999945
262 -0.000500000000000167
263 -0.000529999999999919
264 -0.000529999999999919
265 -0.000539999999999985
266 -0.000530000000000141
267 -0.000539999999999985
268 -0.000539999999999985
269 -0.000539999999999985
270 -0.000529999999999919
271 -0.000530000000000141
272 -0.000530000000000141
273 -0.000529999999999919
274 -0.000529999999999919
275 -0.000529999999999919
276 -0.000520000000000076
277 -0.000520000000000076
278 -0.00051000000000001
279 -0.00051000000000001
280 -0.000489999999999879
281 -0.000530000000000141
282 -0.000520000000000076
283 -0.000520000000000076
284 -0.000520000000000076
285 -0.000519999999999854
286 -0.000529999999999919
287 -0.000529999999999919
288 -0.000539999999999985
289 -0.000539999999999985
290 -0.000539999999999985
291 -0.000529999999999919
292 -0.000519999999999854
293 -0.000519999999999965
294 -0.000509999999999899
295 -0.000539999999999985
296 -0.00051000000000001
297 -0.000519999999999965
298 -0.00051000000000001
299 -0.00051000000000001
300 -0.00052000000000002
301 -0.000519999999999965
302 -0.00051000000000001
303 -0.000499999999999945
304 -0.000500000000000056
305 -0.00051000000000001
306 -0.000509999999999955
307 -0.00054000000000004
308 -0.000549999999999995
309 -0.00053000000000003
310 -0.000560000000000005
311 -0.000520000000000007
312 -0.000539999999999999
313 -0.000519999999999993
314 -0.000510000000000004
315 -0.000519999999999993
316 -0.000530000000000003
317 -0.000519999999999993
318 -0.000520000000000007
319 -0.00052000000000002
320 -0.000519999999999965
321 -0.000529999999999919
322 -0.00053000000000003
323 -0.00051000000000001
324 -0.000519999999999965
325 -0.000519999999999854
326 -0.00051000000000001
327 -0.000530000000000141
328 -0.000519999999999854
329 -0.000529999999999919
330 -0.000510000000000232
331 -0.000520000000000076
332 -0.000519999999999854
333 -0.000520000000000076
334 -0.000549999999999828
335 -0.000529999999999919
336 -0.000519999999999854
337 -0.00051000000000001
338 -0.000500000000000167
339 -0.000499999999999945
340 -0.000519999999999965
341 -0.00048999999999999
342 -0.000490000000000046
343 -0.000480000000000008
344 -0.00048
345 -0.00048
346 -0.00049
347 -0.000479999999999994
348 -0.000480000000000008
349 -0.000479999999999994
350 -0.000479999999999994
351 -0.0005
352 -0.00048999999999999
353 -0.000480000000000008
354 -0.000470000000000026
355 -0.00047999999999998
356 -0.00046999999999997
357 -0.000459999999999988
358 -0.000469999999999998
359 -0.000469999999999998
360 -0.00046
361 -0.000469999999999998
362 -0.000470000000000002
363 -0.000469999999999998
364 -0.000469999999999998
365 -0.000490000000000018
};
\addlegendentry{JPEG50}
\end{axis}

\end{tikzpicture}
